A New Community Definition For MultiLayer Networks And A Novel Approach For Its Efficient Computation

As the use of MultiLayer Networks (or MLNs) for modeling and analysis is gaining popularity, it is becoming increasingly important to propose a community definition that encompasses the multiple features represented by MLNs and develop algorithms for efficiently computing communities on MLNs. Currently, communities for MLNs, are based on aggregating the networks into single graphs using different techniques (type independent, projection-based, etc.) and applying single graph community detection algorithms, such as Louvain and Infomap on these graphs. This process results in different types of information loss (semantics and structure). To the best of our knowledge, in this paper we propose, for the first time, a definition of community for heterogeneous MLNs (or HeMLNs) which preserves semantics as well as the structure. Additionally, our basic definition can be extended to appropriately match the analysis objectives as needed. In this paper, we present a structure and semantics preserving community definition for HeMLNs that is compatible with and is an extension of the traditional definition for single graphs. We also present a framework for its efficient computation using a newly proposed decoupling approach. First, we define a k-community for connected k layers of a HeMLN. Then we propose a family of algorithms for its computation using the concept of bipartite graph pairings. Further, for a broader analysis, we introduce several pairing algorithms and weight metrics for composing binary HeMLN communities using participating community characteristics. Essentially, this results in an extensible family of community computations. We provide extensive experimental results for showcasing the efficiency and analysis flexibility of the proposed computation using popular IMDb and DBLP data sets.

==> texFiles/sc_ProblemStatement.tex <==
\section{Problem Statement}
\label{sec:problem-statement}

%The problem being addressed in this paper can be informally stated as follows. \textit{For a given dataset with M features (explicit or derived) and N entity types along with a set of analysis requirements, i) determine the layers of the homogeneous MLN based on the analysis requirements and ii) develop composition-based community detection algorithms for analysis on arbitrary combinations of layers specified}. Thus, once multiplex layers are created as shown in this paper, any number of analyses can be performed without generating additional graphs/layers. 
We start with a few definitions leading to the formal definition of a community in a MLN.

A graph G = (V, E) is composed of vertices and edges. V is a set of vertices (or nodes) and E $\subseteq$ $V \times V$ is the set of edges of graph G. The size of the graph is defined as the number of vertices of G and it is represented as $|V|$ and the number of edges as $|E|$. If two vertices in G, say \textit{u, v $\in$ V}, are connected by an edge e $\in$ E, this is denoted by \textit{e = (u, v)} and the two vertices are said to be adjacent or neighbors. Edges are said to be undirected when they have no direction. In this paper, all edges are undirected. Note that the above definition does not include multiple edges between nodes, loops, and labels (for both nodes and edges). Our representation and analysis does not require them and we assume unique numbers for nodes across layers.

A multilayer network $MLN (G, X)$, is defined by two sets of single networks. The set $G = \{G_1, G_2, \ldots, G_n\}$ contains general graphs as defined above, where $G_i (V_i, E_i)$ is defined by a set of vertices, $V_i$ and a set of edges, $E_i$. An edge $e(v,u) \in E_i$, connects vertices $v$ and $u$, where $v,u\in V_i$. The set $X =\{X_{1,2}, X_{1,3}, \ldots, X_{n-1,n}\}$ consists of bipartite graphs. Each graph $X_{i,j} (V_i, V_j, L_{i,j})$ is defined by two sets of vertices $V_i$ and $V_j$, and a set of edges (or links) $L_{i,j}$, such that for every link $l(a,b) \in L_{i,j}$,  $a\in V_i$ and $b \in V_j$, where $V_i$ ($V_j$) is the vertex set of graph $G_i$ ($G_j$). 

{\em To summarize}, the set $G$, represents the constituent graphs of layers and the set $X$ represents the graphs that correspond to the edges between a pair of layers. Nodes of X comes from two layers and if labels are assigned, they would have different node labels.

Since we are proposing a decoupling approach for community detection for two layers, we elaborate on our approach below. Figure~\ref{fig:decoupling} shows the approach diagrammatically. Communities for each layer are detected using extant approaches. Layers are then combined pairwise using the bipartite graph approach. Further composition is performed on communities obtained for each layer pair using a join on community identity. The approach is discussed in details in Section~\ref{sec:hemln-community}.

%sc: abhishek, need to slightly modify this fig. drop current approach. show pair-wise composition using bipat approach and join between them.
\begin{wrapfigure}{l}{0.65\textwidth}

   \begin{center}
   \vspace{-30pt}
    \includegraphics[width=0.65\textwidth]{./figures/Decoupling.png}
   \caption{{Current Approach vs Network Decoupling. The difference in pattern in the complete results indicate that the results will be similar, but may not be identical.}}
   \label{fig:decoupling}
\vspace{-10pt}
	\end{center}
\end{wrapfigure}

We define pair-wise network decoupling using two functions (i) $D$, the algorithm for analyzing the constituent networks individually and (ii) $\Theta$, the algorithm for combining the partial results.  Each constituent network, $G_i$, from the heterogeneous multilayer network $N(G,X)$, is analyzed
separately as $D(G_i,X_{i,*})$, where $X_{i,*}$ are the bipartite graphs whose links are connected to $V_i$, to generate the partial results.  The function D is community detection of a single graph corresponding to a layer. The function $\Theta$ is made up og two components: i) the maximum flow algorithm between $G_i$ and any other layer with which  $G_i$ has inter-layer edges and ii) join between communities generated in step i). The paired communities form combined communities between the layers using weights for edges for the bipartite graph based on analysis requirements as discussed in Section~\ref{sec:hemln-community}.

More than two layers are combined using pair-wise communities with a common layer. For example, pair-wise communities for $G_i~and~G_j$ can be joined with pair-wise communities of $G_j~and~G_k$  on community identities of $G_j$. Any number of connected layers can be combined in this way as associativity is satisfied for the join operation.  For a given k layers, the number of pair-wise communities generated as well as the number of join possibilities depends upon the connectivity of layers.

Based on the above, the problem statement can be refined as follows. \textit{For a given dataset with M features (explicit or derived) and N entity types along with a set of analysis requirements,   i) determine the layers of the homogeneous MLN based on the analysis requirements and ii) identify metrics for maximal flow-based bipartite match algorithm and determine the order of joins to form large communities for each analysis.} It is important to note that this formulation of communities preserves entity and feature types as compared to other alternatives proposed in the literature.

Those alternatives are of two kinds: i)  combine (or aggregate) all the layers, ignore types and apply single graph community detection algorithms and ii) projection-based where a layer is projected on to a connected layer as a means of aggregating the two layers and single graph community detection is applied again ignoring entity types.

\sharma{this is a first cut. needs revision and polishing!}

%We express this operation concisely as $D_i$~\footnote{For sake of reducing the number of new terms, we are abusing the notation by representing $D_i$ as both the analysis operation and its corresponding result.}. The partial results are then combined as $D_1 \Theta D_2 \ldots \Theta D_n$. We express this operation concisely as $\Theta_{N}^D$. 


